Event-Based Contrastive Learning for Medical Time Series

In clinical practice, one often needs to identify whether a patient is at high risk of adverse outcomes after some key medical event. For example, quantifying the risk of adverse outcomes after an acute cardiovascular event helps healthcare providers identify those patients at the highest risk of poor outcomes; i.e., patients who benefit from invasive therapies that can lower their risk. Assessing the risk of adverse outcomes, however, is challenging due to the complexity, variability, and heterogeneity of longitudinal medical data, especially for individuals suffering from chronic diseases like heart failure. In this paper, we introduce Event-Based Contrastive Learning (EBCL) - a method for learning embeddings of heterogeneous patient data that preserves temporal information before and after key index events. We demonstrate that EBCL can be used to construct models that yield improved performance on important downstream tasks relative to other pretraining methods. We develop and test the method using a cohort of heart failure patients obtained from a large hospital network and the publicly available MIMIC-IV dataset consisting of patients in an intensive care unit at a large tertiary care center. On both cohorts, EBCL pretraining yields models that are performant with respect to a number of downstream tasks, including mortality, hospital readmission, and length of stay. In addition, unsupervised EBCL embeddings effectively cluster heart failure patients into subgroups with distinct outcomes, thereby providing information that helps identify new heart failure phenotypes. The contrastive framework around the index event can be adapted to a wide array of time-series datasets and provides information that can be used to guide personalized care.

==> Sections/6_Acknowledgements.tex <==
\section{Acknowledgements}
We would like to thank members of the Computational Cardiovascular Research Group and HealthyML Lab at MIT for their invaluable feedback.

==> Sections/Discussion_bk.tex <==
\section{Discussion}
\label{sec:conclusion}

\subsection{Limitations and Future Work}
Our study introduces EBCL, a novel pretraining scheme that demonstrates marked improvements in outcome stratification for heart failure patients through the use of event-centric contrastive learning. While our findings are promising, they are derived from a singular dataset focused on a specific patient cohort, limiting the generalizability of our results. This deliberate focus allowed for a precise evaluation of EBCL within a controlled environment but also highlights the need for broader validation across diverse clinical contexts and datasets to fully understand the method's applicability. The positive results in this context, nonetheless, suggest that EBCL's methodology could be effective more broadly. We remain cautious about extending our claims of effectiveness beyond the current study's scope, but believe our work motivates future experiments applying EBCL to different clinical and non-clinical time series datasets. Additionally, we did not conduct an extensive comparison of more contrastive pretraining methods for windows of time series data or more different model architectures. While further experiments addressing these limitations are important, our current results with several pretraining methods are encouraging.

\section{Conclusion}

In this paper, we propose that EBCL, a novel pretraining scheme for medical time series data, learns patient-specific temporal representations around clinically significant events. We show that EBCL outperforms previous contrastive \citep{agrawal2022leveraging}, generative \cite{labach2023duett, tipirneni2022self}, and supervised baselines through finetuning results in Table \ref{tab:all_results}. We observe that EBCL demonstrates a rich latent space through 1) significant improvement in deep clustering of patients into homogenous outcome clusters and 2) large improvements in classification performance when performing linear probing and KNN classification in the EBCL latent space vs the latent space of baselinemethods. We show through a censoring ablation that the key to EBCL is contrasting local windows, and through event selection ablations that the event selection is vital to the EBCL performance gains. Our method uses a contrastive learning method to address the gaps of generative pretraining methods and induce a deep structure in the latent space \citep{mcdermott2023structure}, additionally we overcome the limitations of applying previous non-event based contrastive learning methods on clinical time series data by focusing on a domain specific event and learning consistent representations around it.

% These strong and promising results merit future evaluation of this method on other clinical index events with similar trends to heart failure. An event, for example, can encompass different clinical occurrences, including episodes of hypoglycemia in diabetic patients, a new diagnosis of hypertension made at an outpatient visit, etc. The key insight is that a key medical event is one where important clinical features change and/or new trends in the patient's clinical trajectory are expected.

% Although we focus our experiments on a heart failure cohort, most, if not all, diseases are similarly punctuated by clinically important events such as Diabetic ketoacidosis complications in patients with type 1 diabetes; sickle cell crises in patients with sickle cell disease, etc. Our method may be appropriate in settings where we have temporal sequences of datasets and knowledge about what types of events are likely to be clinically most meaningful. The primary use case, exemplified in this paper, is to predict cardiovascular outcomes specifically for the heart failure cohort using the in-hospital time-series dataset. For this application, we relied on prior domain knowledge about heart failure in general and its pathophysiology to identify what types of clinical events are likely to be most impactful.

% The method is most appropriate in settings where we have temporal sequences of datasets and some knowledge about what types of events are likely to be clinically most meaningful. The primary use case, exemplified in this paper, is to predict cardiovascular outcomes specifically for the heart failure cohort using the in-hospital time-series dataset. For this application, we relied on prior domain knowledge about heart failure in general and its pathophysiology to identify what types of clinical events are likely to be most impactful.

% The identification of relevant `events' to guide EBCL pretraining need not be restricted to hospital admissions. An event, for example, can encompass different clinical occurrences, including episodes of hypoglycemia in diabetic patients, a new diagnosis of hypertension made at an outpatient visit, etc. The key insight is that a key medical event is one where important clinical features change and/or new trends in the patient's clinical trajectory are expected.  

% We emphasize that the scope of the EBCL model extends well beyond clinical time-series data or specific cohorts like heart failure. Furthermore, the contrastive framework around the index event can be adapted to a wide array of time-series datasets including various modalities including tabular time-series data, time-series of signal, and images by using a multimodal encoder \citep{pmlr-v225-king23a, ghosh2023clipsyntel}. EBCL is designed to be versatile enough to handle multi-modal datasets, making it a comprehensive tool for time-series analysis in diverse modalities and application domains. This flexibility signifies its potential as a universal tool for multi-modal time series.




% In this paper, we propose a novel contrastive learning method, EBCL, and evaluate it on a multi-center cohort of HF patients. We observe significant improvements in finetuning performance compared to baselines, and see even greater improvements in the pretrained embeddings obtained from EBCL

% point 1 - Event based focus is important -- supported by ablations, finetuning, and linear probing results.

% point 2 - EBCL can be extended to other tasks -- this is a weaker point


% EBCL helps address the gaps prior research efforts have left in this critical disease area.

% EBCL, a novel pretraining scheme for medical time series data, learns patient-specific temporal representations around clinically significant events. We show that EBCL outperforms previous contrastive \citep{agrawal2022leveraging}, generative \cite{labach2023duett, tipirneni2022self}, and supervised baselines.

% We evaluate EBCL on a multi-center cohort of heart failure patients. Heart failure is a complex web of disorders, and we have yet to fully understand the full spectrum of subtypes that are observed in heart failure management \cite{borlaug2020evaluation, shah2016phenotype}. Methods that can identify meaningful subtypes with different levels of risk can help to enhance the discovery of personalized therapies that are appropriate for a given patient's risk \cite{afsin2015diagnosis}. However, existing methods for phenotyping heart failure \cite{ahmad2018machine, shah2015phenomapping, meijs2023discovering} do not fully utilize the rich and heterogeneous nature of time-series data in clinical settings.


% Although we focus our experiments on a heart failure cohort, most, if not all, diseases are similarly punctuated by clinically important events such as Diabetic ketoacidosis complications in patients with type 1 diabetes; sickle cell crises in patients with sickle cell disease, etc. Our method is appropriate in settings where we have temporal sequences of datasets and knowledge about what types of events are likely to be clinically most meaningful. The primary use case, exemplified in this paper, is to predict cardiovascular outcomes specifically for the heart failure cohort using the in-hospital time-series dataset. For this application, we relied on prior domain knowledge about heart failure in general and its pathophysiology to identify what types of clinical events are likely to be most impactful.


% In conclusion, EBCL represents a significant advancement in the utilization of medical time series data for patient care. By effectively capturing and analyzing the temporal nuances of patient trajectories, EBCL paves the way for more personalized, predictive, and preventative healthcare strategies. Our contributions lay the groundwork for further exploration and application of contrastive pretraining methods in medicine, promising to enhance patient outcomes and healthcare delivery across various domains, as evidenced by its ability to outperform established pretraining methods in linear probing evaluations and its potential for patient subtyping \cite{afsin2015diagnosis, Jafari2020, Gheorghiade2005, Collins2019, borlaug2020evaluation, shah2016phenotype}.

% Methods that can identify meaningful subtypes with different levels of risk can help to enhance the discovery of personalized therapies that are appropriate for a given patient's risk \cite{afsin2015diagnosis}. Such a tailored methodology not only provides a deeper understanding of each patient's unique condition but also opens the door to more effective and efficient healthcare solutions. However, existing methods for phenotyping heart failure \cite{ahmad2018machine, shah2015phenomapping, meijs2023discovering} do not fully utilize the rich and heterogeneous nature of time-series data in clinical settings.

% Patient subtyping into groups with similar outcomes can help discover subgroups of patients that respond well to similar treatments \citep{afsin2015diagnosis}. Subtyping can help physicians to administer preventative treatments, and improve patient care \citep{Jafari2020}.Our pretraining method is able to learn more outcome homogenous clusters of patients, suggesting the potential application of our method for improving heart failure subtyping.

% In this application we apply our approach to a cohort of heart failure, where a hospital admission is the clinically significant event of interest. Heart failure provides a particularly good application domain because the trajectory of patients with heart failure is punctuated by frequent hospital admissions, where each admission is associated with a further decrease in myocardial function \citep{Gheorghiade2005}; i.e., hospital admissions are particularly important in the health trajectory of these patients.  

% EBCL, a novel pretraining scheme for medical time series data, learns patient-specific temporal representations around clinically significant events. We show that EBCL outperforms previous contrastive \citep{agrawal2022leveraging}, generative \cite{labach2023duett, tipirneni2022self}, and supervised baselines.

% The trajectory of patients with heart failure is punctuated by frequent hospital admissions, where each admission is associated with a further decrease in myocardial function \citep{Gheorghiade2005}. The ability to identify patients at high risk of readmission or death forms an integral part of their evaluation and care \citep{Collins2019}. EBCL explicitly models such temporal information around important clinical events.

% The identification of relevant `events' to guide EBCL pretraining need not be restricted to hospital admissions. An event, for example, can encompass different clinical occurrences, including episodes of sepsis onset in intensive care unit patients \citep{johnson2023mimic}, hypoglycemia in diabetic patients, a new diagnosis of hypertension made at an outpatient visit, vaccination of COVID-19 patients \cite{Wahltinez2020}, etc. The key insight is that a key medical event is one where important clinical features change and/or new trends in the patient's clinical trajectory are expected.  

% We emphasize that the scope of the EBCL model extends well beyond clinical time-series data or specific cohorts like heart failure. Furthermore, the contrastive framework around the index event can be adapted to a wide array of time-series datasets including various modalities including tabular time-series data, time-series of signal, and images by using a multimodal encoder \citep{pmlr-v225-king23a, ghosh2023clipsyntel}. EBCL is designed to be versatile enough to handle multi-modal datasets, making it a comprehensive tool for time-series analysis in diverse modalities and application domains. This flexibility signifies its potential as a universal tool for multi-modal time series.

%### Add to the Discussion

% \citep{hernandez2010relationship, pandey2016association, bradley2013hospital, tung2016worse}
% \citep{subramanian2011new, spertus2003challenges,gupta2018association,ouwerkerk2014factors}

\section{Broader Impact}
This paper presents EBCL, aiming to make significant contributions to healthcare, particularly in enhancing risk stratification for heart failure patients using extensive time series data from a major tertiary hospital. The potential positive impacts of EBCL are considerable and varied. Firstly, by automatically identifying high-risk patients at discharge, EBCL stands to substantially improve patient care, potentially leading to fewer hospital readmissions and enhanced patient outcomes \citep{rahimi2014risk}. Secondly, EBCL's advanced prediction models could facilitate the optimal allocation of healthcare resources, ensuring timely care for high-risk patients \citep{duong2021identification, jencks2009rehospitalizations}. This shift towards more preventive care strategies could help mitigate the need for more intensive, and often expensive, interventions later on \citep{Jafari2020}. Lastly, EBCL introduces methodological innovations that simplify the incorporation of domain expertise into the pretraining process through the selection of index events. This approach not only enhances the application of EBCL to complex time series data but also opens avenues for its adoption across various other domains, demonstrating the method's versatility and potential for broad impact.
% Patient subtyping into groups with similar outcomes can help discover subgroups of patients that respond well to similar treatments \citep{afsin2015diagnosis}. Subtyping can help physicians to administer preventative treatments, and improve patient care \citep{Jafari2020}

However, the application of EBCL raises important ethical considerations and potential societal consequences. The use of patient data, even in de-identified form, necessitates stringent adherence to data privacy and security standards such as those outlined by HIPAA \cite{dwyer2004health} in the United States. Moreover, there is a critical need to address and mitigate biases within machine learning models to prevent the perpetuation of inequalities in healthcare access and outcomes \citep{Ganapathi2022, Obermeyer2019}. Such biases could otherwise limit the benefits of these technologies to certain patient groups, and we must scrutinize and adapt models prior to deployment to avoid this.


% In this study, we introduce EBCL, a novel pretraining approach tailored for medical time series data, focusing on learning patient-specific temporal trends around clinically significant events. Our evaluation, centered on a heart failure cohort, demonstrates EBCL's superiority over existing pretraining, generative, and supervised learning methods in predicting three critical cardiovascular outcomes. This focused analysis reveals EBCL's potential to leverage clinically significant events to improve downstream task performance for a specific patient population.

% We acknowledge that our study evaluates EBCL within a singular context: a specific dataset, a single patient cohort, and a limited set of outcomes. 
% This focused approach was chosen to meticulously assess EBCL's performance in a well-defined setting, providing a clear indication of its potential benefits. However, this also constitutes a limitation, as the findings are based on a single source and population.
% The positive results in this context suggest that EBCL's methodology, which leverages temporal sequences and domain-specific events, could be effective more broadly. We remain cautious about extending our claims of effectiveness beyond the current study's scope, and believe our work motivates future experiments applying EBCL to different clinical and non-clinical time series datasets.

% Given the promising performance of EBCL in this heart failure cohort, expanding the application of EBCL to other clinical conditions, datasets, and outcomes is necessary to understand its strengths and limitations. The simplicity of contrasting around index events allows the EBCL framework to be easily formulated for other ??? suggests its adaptability to various medical events and conditions, yet the extent of its efficacy in different contexts remains to be explored.



%  We demonstrate its effectiveness compared to other pretraining and supervised baselines in learning patient-specific temporal representations for predicting cardiovascular outcomes in a heart failure cohort. Our approach leverages clinically significant events to guide the learning process, a methodology that showed promise in the context of our focused application.
 
% While our findings are encouraging, it's important to note the study's limitations, including its reliance on evaluating using three outcomes on a single dataset and cohort. Further research to explore EBCL's applicability to other clinical scenarios is necessary, and future studies may investigate EBCL's potential in other clinical and nonclinical time series settings.

==> Sections/Table2_Results_prev.tex <==
\begin{table*}[h!]
\caption{\textbf{EBCL Pretraining improves results over a supervised baseline and time-series pretraining baselines in the Heart Failure Dataset.} We summarize the downstream finetuning performance using both the area under the receiver operating characteristic (AUC) and the area under the precision-recall curve (APR) of three prediction tasks (30-Day Readmission, 1-Year Mortality, and 1-Week Length of Stay (LOS)) averaged over 5 runs with different seeds. Across all tasks, EBCL results (boldfaced) were statistically significantly better than all other tested models.
}
\label{tab:pred}
\footnotesize
\begin{center}
  \begin{tabular}{lcccccc}
  \toprule
    & \multicolumn{2}{c}{30-Day Readmission} &\multicolumn{2}{c}{1-Year Mortality} &\multicolumn{2}{c}{1-Week LOS} \\
    \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}
    & AUC & APR  & AUC & APR & AUC & APR \\
    \midrule
    XGBoost
    & 70.85 $\pm$ 0.08
    & 86.19 $\pm$ 0.03
    & 80.33 $\pm$ 0.19
    & 89.58 $\pm$ 0.08
    & 79.74 $\pm$ 0.10
    & 79.79 $\pm$ 0.08
    \\
    S-Trans
    & 70.28 $\pm$ 0.16
    & 85.60 $\pm$ 0.12
    & 81.54 $\pm$ 0.24
    & 90.27 $\pm$ 0.15
    & 88.74 $\pm$ 0.48
    & 88.61 $\pm$ 0.48
    \\
    \midrule
    OCP %\cite{agrawal2022leveraging}
    & 70.27 $\pm$ 0.32
    & 85.48 $\pm$ 0.20
    & 80.06 $\pm$ 0.29
    & 89.36 $\pm$ 0.18
    & 90.06 $\pm$ 0.25
    & 90.05 $\pm$ 0.28
    \\
    STraTS %\cite{tipirneni2022self}
    & 70.06 $\pm$ 0.11
    & 85.45 $\pm$ 0.07
    & 79.95 $\pm$ 0.62
    & 89.31 $\pm$ 0.43
    & 88.36 $\pm$ 1.09
    & 87.73 $\pm$ 2.03
    \\
    DueTT %\cite{labach2023duett}
    & 69.51 $\pm$ 0.50
    & 85.51 $\pm$ 0.31
    & 79.39 $\pm$ 0.16
    & 89.04 $\pm$ 0.11
    & 75.35 $\pm$ 0.61 % 75.98$\pm$
    & 74.66 $\pm$ 0.62 % 75.22$\pm$
    \\
    \midrule
    EBCL
    & \textbf{71.66 $\pm$ 0.03}
    & \textbf{86.40 $\pm$ 0.03}
    & \textbf{82.43 $\pm$ 0.07}
    & \textbf{90.55 $\pm$ 0.03}
    & \textbf{90.98 $\pm$ 0.05}
    & \textbf{90.96 $\pm$ 0.04}
    \\
    \bottomrule
\end{tabular}
\end{center}
\end{table*}

%0.7598211765	0.388101	0.692676723	0.5697187781

